Counting smaller elements in the Tamari and m-Tamari lattices

We introduce new combinatorial objects, the interval- posets, that encode intervals of the Tamari lattice. We then find a combinatorial interpretation of the bilinear operator that appears in the functional equation of Tamari intervals described by Chapoton. Thus, we retrieve this functional equation and prove that the polynomial recursively computed from the bilinear operator on each tree T counts the number of trees smaller than T in the Tamari order. Then we show that a similar m + 1-linear operator is also used in the functionnal equation of m-Tamari intervals. We explain how the m-Tamari lattices can be interpreted in terms of m+1-ary trees or a certain class of binary trees. We then use the interval-posets to recover the functional equation of m-Tamari intervals and to prove a generalized formula that counts the number of elements smaller than or equal to a given tree in the m-Tamari lattice.

==> figures/composition.tex <==

\def \fpath{figures/interval-posets/}
\def \sscale{0.6}

\begin{align*}
\BB( 
\begin{aligned}
\scalebox{\sscale}{\input{\fpath I3-ex3}}
\end{aligned}
,
\begin{aligned}
\scalebox{\sscale}{\input{\fpath I4-ex1}}
\end{aligned}
)
&=
\begin{aligned}
\scalebox{\sscale}{\input{\fpath I8-ex1}}
\end{aligned}
+
\begin{aligned}
\scalebox{\sscale}{\input{\fpath I8-ex2}}
\end{aligned} \\
&+ 
\begin{aligned}
\scalebox{\sscale}{\input{\fpath I8-ex3}}
\end{aligned}
+ 
\begin{aligned}
\scalebox{\sscale}{\input{\fpath I8-ex4}}
\end{aligned}
\end{align*}


==> figures/interval-posets/I2-ex1.tex <==
% Auteur : Viviane Pons
% Création : 16/05/2013


\begin{tikzpicture}[scale=0.8]
\node(T1) at (0,0) {1};
\node(T2) at (0,-1) {2};
\draw[line width = 0.5, color=red] (T2) -- (T1);
\end{tikzpicture}



==> figures/interval-posets/I3-ex4.tex <==
% Auteur : Viviane Pons
% Création : 16/05/2013

\def \wlev{0.5}
\def \hlev{0.8}

\begin{tikzpicture}

\node(N1) at (0,\hlev) {1};
\green{
\node(T1) at (0,0) {2};
\node(T2) at (0,-1) {3};
\draw[line width = 0.5, color=red] (T2) -- (T1);
}
\end{tikzpicture}


==> figures/interval-posets/I3-ex5.tex <==
% Auteur : Viviane Pons
% Création : 16/05/2013

\def \wlev{0.5}
\def \hlev{0.8}

\begin{tikzpicture}

\node(N1) at (0,\hlev) {1};
\green{
\node(T1) at (0,0) {2};
\node(T2) at (0,-1) {3};
\draw[line width = 0.5, color=red] (T2) -- (T1);
}
\draw[line width = 0.5, color=red](T1) -- (N1);
\end{tikzpicture}


==> figures/interval-posets/I4-ex2.tex <==
% Auteur : Viviane Pons
% Création : 10/05/2013

\def \wlev{0.5}
\def \hlev{0.8}

\begin{tikzpicture}[scale=0.8]
\node(T2) at (0,-1) {2};
\node(T1) at (0,0) {1};
\node(T3) at (1,-1) {3};
\node(T4) at (1,-2) {4};
\draw[line width = 0.5, color=blue] (T2) -- (T3);
\draw[line width = 0.5, color=red] (T2) -- (T1);
\draw[line width = 0.5, color=red] (T4) -- (T3);
\end{tikzpicture}



==> figures/interval-posets/I6-ex1.tex <==
% Auteur : Viviane Pons
% Création : 10/05/2013
\def \hlev{0.8}
\def \wlev{0.6}

\begin{tikzpicture}
\node(N1) at (0,0) {1};
\node(N2) at (0.5 * \wlev,-1 * \hlev) {2};
\node(N3) at (\wlev,0) {3};
\node(N4) at (2 * \wlev,0) {4};
\node(N5) at (3 * \wlev,0) {5};
\node(N6) at (3 * \wlev,-1 * \hlev) {6};
\draw (N2) -- (N3);
\draw (N2) -- (N1);
\draw (N6) -- (N5);
\end{tikzpicture}


==> figures/interval-posets/I6-ex6.tex <==


\begin{tikzpicture}[scale=1]
\node(T1) at (0,0) {1};
\node(T2) at (0,-1) {2};
\node(T3) at (1,0) {3};
\node(T4) at (2,0) {4};
\node(T5) at (1,-1) {5};
\node(T6) at (2,-1) {6};
\draw[line width = 0.5, color=blue] (T1) -- (T3);
\draw[line width = 0.5, color=blue] (T2) -- (T3);
\draw[line width = 0.5, color=blue] (T3) -- (T4);
\draw[line width = 0.5, color=blue] (T5) -- (T6);
\end{tikzpicture}

==> figures/mcomposition.tex <==
% Auteur : Viviane Pons
% Création : 16/05/2013
% Modifications : 17/05/2013

\def \fpath{figures/interval-posets/}
\def \sscale{0.6}

\begin{align}
\BBk{2} \left( 
\begin{aligned}\blue{\scalebox{\sscale}{\input{\fpath I2-ex1}}}\end{aligned},
\begin{aligned}\red{\scalebox{\sscale}{\input{\fpath I4-ex2}}}\end{aligned},
\begin{aligned}\green{\scalebox{\sscale}{\input{\fpath I2-ex1}}}\end{aligned}
\right) &=
\begin{aligned}\blue{\scalebox{\sscale}{\input{\fpath I2-ex1}}}\end{aligned} \pleft
\left(
u \prightx \left( 
\left( u \pright \begin{aligned}\green{\scalebox{\sscale}{\input{\fpath I2-ex1}}}\end{aligned} \right) 
\pleft
\begin{aligned}\red{\scalebox{\sscale}{\input{\fpath I4-ex2}}}\end{aligned} \right) 
\right)
\end{align}
\begin{align*}
u \pright \begin{aligned}\green{\scalebox{\sscale}{\input{\fpath I2-ex1}}}\end{aligned} &= 
\begin{aligned}\scalebox{\sscale}{\input{\fpath I3-ex4}}\end{aligned}
+ \begin{aligned}\scalebox{\sscale}{\input{\fpath I3-ex5}}\end{aligned} \\
\left( u \pright \begin{aligned}\green{\scalebox{\sscale}{\input{\fpath I2-ex1}}}\end{aligned} \right)
\pleft
\begin{aligned}\red{\scalebox{\sscale}{\input{\fpath I4-ex2}}}\end{aligned} &=
 \begin{aligned}\scalebox{\sscale}{\input{\fpath I7-ex1}}\end{aligned}
+  \begin{aligned}\scalebox{\sscale}{\input{\fpath I7-ex2}}\end{aligned}
\end{align*}
\begin{align}
\label{eq:mtamari:exemple-prightx}
u \prightx \left( 
\left( u \pright \begin{aligned}\green{\scalebox{\sscale}{\input{\fpath I2-ex1}}}\end{aligned} \right) 
\pleft
\begin{aligned}\red{\scalebox{\sscale}{\input{\fpath I4-ex2}}}\end{aligned} \right) &=
\begin{aligned}\scalebox{\sscale}{\input{\fpath I8-ex5}}\end{aligned}
+ \begin{aligned}\scalebox{\sscale}{\input{\fpath I8-ex6}}\end{aligned}
+ \begin{aligned}\scalebox{\sscale}{\input{\fpath I8-ex7}}\end{aligned}
+ \begin{aligned}\scalebox{\sscale}{\input{\fpath I8-ex8}}\end{aligned} \\
\notag
&+ \begin{aligned}\scalebox{\sscale}{\input{\fpath I8-ex9}}\end{aligned}
+ \begin{aligned}\scalebox{\sscale}{\input{\fpath I8-ex10}}\end{aligned}
+ \begin{aligned}\scalebox{\sscale}{\input{\fpath I8-ex11}}\end{aligned}
\end{align}
\begin{align}
\label{eq:mtamari:exemple-mcomp}
\BBk{2} \left( 
\begin{aligned}\blue{\scalebox{\sscale}{\input{\fpath I2-ex1}}}\end{aligned},
\begin{aligned}\red{\scalebox{\sscale}{\input{\fpath I4-ex2}}}\end{aligned},
\begin{aligned}\green{\scalebox{\sscale}{\input{\fpath I2-ex1}}}\end{aligned}
\right) &=
\begin{aligned}\scalebox{\sscale}{\input{\fpath I10-ex1}}\end{aligned}
+ \begin{aligned}\scalebox{\sscale}{\input{\fpath I10-ex2}}\end{aligned}
+ \begin{aligned}\scalebox{\sscale}{\input{\fpath I10-ex3}}\end{aligned}
+ \begin{aligned}\scalebox{\sscale}{\input{\fpath I10-ex4}}\end{aligned} \\
\notag
& + \begin{aligned}\scalebox{\sscale}{\input{\fpath I10-ex5}}\end{aligned}
+ \begin{aligned}\scalebox{\sscale}{\input{\fpath I10-ex6}}\end{aligned}
+ \begin{aligned}\scalebox{\sscale}{\input{\fpath I10-ex7}}\end{aligned}
\end{align}

==> figures/trees/T3-1-n.tex <==
% Auteur : Viviane Pons
% Création 27/04/2013

%       .
%     ./
%   ./

\begin{tikzpicture}
\node (N0) at (2.500, 0.000){3};
\node (N00) at (1.500, -1.000){2};
\node (N000) at (0.500, -2.000){1};
\draw (N00) -- (N000);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T3-2-n.tex <==
% Auteur : Viviane Pons
% Création 27/04/2013

%       .
%     ./
%      \.

\begin{tikzpicture}
\node (N0) at (2.500, 0.000){3};
\node (N00) at (0.500, -1.000){1};
\node (N001) at (1.500, -2.000){2};
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T3-3-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%        \.
%       ./

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (2.500, -1.000){3};
\node (N010) at (1.500, -2.000){2};
\draw (N01) -- (N010);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T3-5-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%       .
%        \.
%          \.

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (1.500, -1.000){2};
\node (N011) at (2.500, -2.000){3};
\draw (N01) -- (N011);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-1-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%      /
%     /
%    /

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (2.500, -1.000){3};
\node (N000) at (1.500, -2.000){2};
\node (N0000) at (0.500, -3.000){1};
\draw (N000) -- (N0000);
\draw (N00) -- (N000);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T4-10-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%        .
%         \.
%        ./
%      ./

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (3.500, -1.000){4};
\node (N010) at (2.500, -2.000){3};
\node (N0100) at (1.500, -3.000){2};
\draw (N010) -- (N0100);
\draw (N01) -- (N010);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-11-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%        .
%         \.
%        ./
%         \.

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (3.500, -1.000){4};
\node (N010) at (1.500, -2.000){2};
\node (N0101) at (2.500, -3.000){3};
\draw (N010) -- (N0101);
\draw (N01) -- (N010);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-13-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%        .
%         \.
%           \.
%          ./

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (1.500, -1.000){2};
\node (N011) at (3.500, -2.000){4};
\node (N0110) at (2.500, -3.000){3};
\draw (N011) -- (N0110);
\draw (N01) -- (N011);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-14-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%         \.
%           \.
%             \.

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (1.500, -1.000){2};
\node (N011) at (2.500, -2.000){3};
\node (N0111) at (3.500, -3.000){4};
\draw (N011) -- (N0111);
\draw (N01) -- (N011);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-2-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%      ./
%    ./
%     \

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (2.500, -1.000){3};
\node (N000) at (0.500, -2.000){1};
\node (N0001) at (1.500, -3.000){2};
\draw (N000) -- (N0001);
\draw (N00) -- (N000);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T4-3-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%      ./
%    ./\.

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (1.500, -1.000){2};
\node (N000) at (0.500, -2.000){1};
\node (N001) at (2.500, -2.000){3};
\draw (N00) -- (N000);
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T4-4-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%      ./
%       \.
%      ./

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (0.500, -1.000){1};
\node (N001) at (2.500, -2.000){3};
\node (N0010) at (1.500, -3.000){2};
\draw (N001) -- (N0010);
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T4-5-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%        .
%      ./
%       \.
%        \.

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (0.500, -1.000){1};
\node (N001) at (1.500, -2.000){2};
\node (N0011) at (2.500, -3.000){3};
\draw (N001) -- (N0011);
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T4-8-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%      ./ \.
%        ./

\begin{tikzpicture}
\node (N0) at (1.500, 0.000){2};
\node (N00) at (0.500, -1.000){1};
\node (N01) at (3.500, -1.000){4};
\node (N010) at (2.500, -2.000){3};
\draw (N01) -- (N010);
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-9-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%      ./ \.
%           \.

\begin{tikzpicture}
\node (N0) at (1.500, 0.000){2};
\node (N00) at (0.500, -1.000){1};
\node (N01) at (2.500, -1.000){3};
\node (N011) at (3.500, -2.000){4};
\draw (N01) -- (N011);
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}
